Quality Assessment of Tabular Data using Large Language Models and Code Generation

Reliable data quality is crucial for downstream analysis of tabular datasets, yet rule-based validation often struggles with inefficiency, human intervention, and high computational costs. We present a three-stage framework that combines statistical inliner detection with LLM-driven rule and code generation. After filtering data samples through traditional clustering, we iteratively prompt LLMs to produce semantically valid quality rules and synthesize their executable validators through code-generating LLMs. To generate reliable quality rules, we aid LLMs with retrieval-augmented generation (RAG) by leveraging external knowledge sources and domain-specific few-shot examples. Robust guardrails ensure the accuracy and consistency of both rules and code snippets. Extensive evaluations on benchmark datasets confirm the effectiveness of our approach.

==> latex/figures/acl_DQ_rules_table.tex <==
\begin{table*}[ht!]
\centering
\resizebox{0.8\textwidth}{!}{%  
\begin{tabular}{||p{2.4cm}||p{4.4cm}|p{8.5cm}||}
\hline
\textbf{DQ Dimension}        & \textbf{DQ Rule Type}                 & \textbf{Sample DQ Rules (Rule Cards)}  \\
\hline
\multirow{1}{*}{Accuracy}  & Reference Table Verification & \\
\hline
\multirow{4}{*}{Conformity}  & Format Compliance                     & 
$\forall x \in \texttt{journal\_issn} \newline
\quad x \models \texttt{[0-9]\{4\}-[0-9]\{3\}[0-9X]}
$ \\ \cline{2-3} 
                             & Data Type Validation                  & $\forall x \in \texttt{article\_jvolume},\quad x \in \mathbb{Z}
$ \\ \cline{2-3} 
                             & \multirow{2}{*}{Pattern Matching}     & $\forall x \in \texttt{article\_pagination},\quad x \models \texttt{[0-9]+\text{-}[0-9]+}$                                                                            \\ \cline{3-3} 
                             &                                       & $\forall x \in \texttt{article\_language},\quad x \models \texttt{[a-z]\{3\}}$  \\ 
\hline
\multirow{1}{*}{Completeness}  & Missing Value Identification & \\
\hline
\multirow{4}{*}{Consistency}                    & \multirow{3}{*}{Value Set Constraint}    & $\forall i \in \{1, \dots, n\}, \newline \quad \text{Genre}_i \subseteq \{\text{Horror}, \text{Comedy}, \text{Drama}, \text{Action}, \text{Romance}..\}$  \\ \cline{3-3}
                                                &                                          & $\forall i \in \{1, \dots, n\}, \newline \quad \text{Language}_i \subseteq \{\text{English}, \text{French}, \text{Spanish}, \text{Dutch}...\}$   \\ \cline{3-3}
                                                &                                          & $\forall i \in \{1, \dots, n\}, \newline \quad \text{Country}_i \subseteq \{\text{USA}, \text{UK}, \text{Netherlands}, \text{France}, \text{Germany}\}$   \\ \cline{2-3} 
                                                & \multirow{2}{*}{Cross-Column Validation} & $\forall i \in \{1, \dots, n\}, \newline \quad
\text{if } \text{Genre}_i \ni \text{Documentary} \Rightarrow \text{Duration}_i \leq 120$                                              \\ \cline{3-3} 
                                                &                                          & $\forall i \in \{1, \dots, n\}, \newline \quad
\left\{
\begin{array}{ll}
\text{if } \text{has\_child}_i = 'Y' \Rightarrow \text{child\_exemp}_i > 0 \\
\text{if } \text{has\_child}_i = 'N' \Rightarrow \text{child\_exemp}_i = 0 \\
\text{child\_exemp}_i < \min(\text{single}_i, \text{married}_i)
\end{array}
\right.$                                              \\ \hline
\multirow{2}{*}{Validity}                    & \multirow{2}{*}{Dependency Constraints}                                              & $order\_status == \text{'Returned'} \Rightarrow return\_initiation\_date \neq \text{NULL}$                         \\ 
                                                \hline
\end{tabular}}
\caption{Examples of DQ Rules categorized by different DQ Dimensions (additional Rules in Appendix \ref{sec:additional_rule_types}). Format Compliance, Data Type Validation and Pattern Matching is using Rayyan and rest using Movies dataset.}
\label{tab:dq_rules}
\end{table*}

==> latex/figures/draft_and_enriched_rule_beers.tex <==
\begin{figure}[ht!]
    \tiny
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\parskip}{0pt}
    \centering
    \begin{tcolorbox}[
        colback=orange!3!white,
        colframe=orange!45!white,
        title=\textcolor{black}{Rule Card (example)},
        boxsep=1pt,
        left=2pt,
        right=2pt,
        top=2pt,
        bottom=0pt,
        width=\linewidth
    ]
        \begin{verbatim}
{
    "Rule Type": "Reference Type Verification",
    "Rule Name": "State Must Be Valid U.S. Abbreviation",
    "Rule Description": "The state column value must exist in the state_id
    field of states.csv (external_knowledge_base/states). Any value not
    found in that reference list is invalid.",
    "Target Columns": [
        "state"
    ],
    "Reference Table": "states.csv"
}
    \end{verbatim}
    \end{tcolorbox}
    \caption{\textit{Rule Card} generated by Gemma-3-12B on Beers dataset \cite{Beers.dataset}.}
    \label{fig:beers_example_rule_card}
\end{figure}


\begin{figure}[ht!]
    \tiny
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\parskip}{0pt}
    \centering
    \begin{tcolorbox}[
        colback=blue!3!white,
        colframe=blue!45!white,
        title=\textcolor{black}{Rule Card (enriched)},
        boxsep=1pt,
        left=2pt,
        right=2pt,
        top=2pt,
        bottom=0pt,
        width=\linewidth
    ]
        \begin{verbatim}

{
    "Rule Type": "Reference Type Verification",
    "Rule Name": "State Must Be Valid U.S. Abbreviation",
    "Rule Description": "The state column value must exist in the state_id     
    field of states.csv (external_knowledge_base/states).
    Any value not found in that reference list is 
    invalid.",
    "Target Columns": [
        "state"
    ],
    "Reference Table": "states.csv"
    "Additional Information": {
        "Specification": "The `state` column value must exist in the 
        `states.csv` reference table.",
        "Pseudocode": [
            "if state is null -> flag",
            "if state is not in states.csv -> flag"
        ]
    }
}
    \end{verbatim}
    \end{tcolorbox}
    \caption{Rule Card enriched by Gemma-3-12B on Beers dataset \cite{Beers.dataset}.}
    \label{fig:enrichered_beer_example_rule_card}
\end{figure}
